Global Convergence Analysis of the Power Proximal Point and Augmented Lagrangian Method

In this paper we study an unconventional inexact Augmented Lagrangian Method (ALM) for convex optimization problems, as first proposed by Bertsekas, wherein the penalty term is a potentially non-Euclidean norm raised to a power between one and two. We analyze the algorithm through the lens of a nonlinear Proximal Point Method (PPM), as originally introduced by Luque, applied to the dual problem. While Luque analyzes the order of local convergence of the scheme with Euclidean norms our focus is on the non-Euclidean case which prevents us from using standard tools for the analysis such as the nonexpansiveness of the proximal mapping. To allow for errors in the primal update, we derive two implementable stopping criteria under which we analyze both the global and the local convergence rates of the algorithm. More specifically, we show that the method enjoys a fast sublinear global rate in general and a local superlinear rate under suitable growth assumptions. We also highlight that the power ALM can be interpreted as classical ALM with an implicitly defined penalty-parameter schedule, reducing its parameter dependence. Our experiments on a number of relevant problems suggest that for certain powers the method performs similarly to a classical ALM with fine-tuned adaptive penalty rule, despite involving fewer parameters.

==> proofs/global_subgradient.tex <==
\begin{proof}
From \cref{alg:inexact_pppa_averaging} we have that $v^k \in \partial_{\varepsilon_k}(y^{k+1})$ and $y^{k+1} = y^k - \lambda \nabla \phi^*(v^k)$.
In light of \cref{thm:decrease_inexact_ppa} we have for any $y \in \bR^m$:
\begin{align} \label{eq:decrease_inexact_ppa}
    \phi(y^{k+1}) \leq \phi(y) + \lambda \star \phi(y^k-y) + \varepsilon_k.
\end{align}
Now consider an arbitrary increasing sequence $\{A_k\}_{k=0}^\infty$ with $A_k >0$ and $A_0=0$. We define $a_{k+1} := A_{k+1} - A_k$.

Plugging $y := \tfrac{a_{k+1} y^\star + A_k y^k}{A_{k+1}}$ in the inequality above we obtain by convexity of $\phi$ since $y^k-y=\tfrac{a_{k+1}}{A_{k+1}}(y^k-y^\star)$ using the positive homogeneity of $\phi$ with order $p+1$
\begin{align*}
    \phi(y^{k+1}) \leq \tfrac{a_{k+1}}{A_{k+1}}\phi(y^\star) + \tfrac{A_{k}}{A_{k+1}}\phi(y^k) + (\tfrac{a_{k+1}}{A_{k+1}})^{p+1}(\lambda \star \phi)(y^k-y^\star) + \varepsilon_k.
\end{align*}
Multiplying both sides with $A_{k+1}$ we get since $a_{k+1}= A_{k+1} - A_k$
\begin{align*}
    A_{k+1}\big(\phi(y^{k+1})-\phi(y^\star)\big) \leq A_{k}\big(\phi(y^k)-\phi(y^\star)\big) +  \tfrac{a_{k+1}^{p+1}}{A_{k+1}^p}(\lambda \star\phi)(y^k-y^\star) + \varepsilon_k A_{k+1}.
\end{align*}
Summing the inequality from $k=0$ to $k=K-1$ we obtain since $A_0 = 0$:
\begin{align} \label{eq:decrease_inexact_ppa_main}
    A_{K}\big(\phi(y^{K}) - \phi(y^\star)\big) \leq \sum_{k=0}^{K-1} \tfrac{a_{k+1}^{p+1}}{A_{k+1}^p}(\lambda \star \phi)(y^k-y^\star) + \varepsilon_k A_{k+1}.
\end{align}
Choosing $y=y^k$ in \cref{eq:decrease_inexact_ppa} we have $\phi(y^{k+1}) \leq \phi(y^k)+ \varepsilon_k.$
Summing the inequality from $k=0$ to $k=K-1$ we obtain $
    \phi(y^{K})-\phi(y^0) \leq \sum_{k=0}^{K-1}\varepsilon_k \leq \beta,$
and hence $\|y^K-y^\star\| \leq D_\beta$ for any $K \geq 0$. This implies that $\phi(y^k-y^\star) =\tfrac{1}{p+1}\|y^\star - y^k\|^{p+1} \leq \tfrac{1}{p+1}D_\beta^{p+1}$.
Thus we can further bound \cref{eq:decrease_inexact_ppa_main}:
\begin{align*} 
    A_{K}\big(\phi(y^{K}) - \phi(y^\star)\big) \leq \lambda^{-p}\tfrac{1}{p+1}D_\beta^{p+1} \sum_{k=1}^{K} \tfrac{a_{k}^{p+1}}{A_{k}^p} + \varepsilon_k A_{k+1}.
\end{align*}
We choose $A_{K}=K^{p+1}$ and by using the fact that $\sum_{k=1}^{K} \tfrac{a_{k}^{p+1}}{A_{k}^p} \leq (p+1)^{p+1}K$ we get:
\begin{align*} 
    A_{K}\big(\phi(y^{K}) - \phi(y^\star)\big) \leq \lambda^{-p}D_\beta^{p+1} (p+1)^{p}K + c K.
\end{align*}
Dividing by $A_K$ we obtain $\phi(y^{K}) - \phi(y^\star) \leq \tfrac{\lambda^{-p}D_\beta^{p+1} (p+1)^{p} + c}{K^p}.$
\ifx\ifsvjour\true
\qed
\fi
\end{proof}

==> proofs/joint_complexity.tex <==
In light of \cref{thm:alm-linear-ergodic} we have that 
$$
\max\{\|A\breve x^K - b\|_*, |f(\breve x^{K}) - f(x^\star)|\} \leq \tfrac{c + \max_{y \in \delta \mathcal{B}}\lambda \star \phi(y^0-y)(p+1)^{p+1}}{K^{p}}.
$$
Since we ask for the total number of iterations such that $\max\{\|A\breve x^K - b\|_*, |f(\breve x^{K}) - f(x^\star)|\} \leq \varepsilon$ and choose $\lambda = \max_{y \in \delta \mathcal{B}}\phi(y^0-y)^q(p+1)^{1+q}$ the total number of outer iterations $K$ is lower-bounded by $(\tfrac{c+1}{\varepsilon})^q$. Let $K$ then be the first integer after $(\tfrac{c+1}{\varepsilon})^q$. Note that the total number of iterations required to obtain $\varepsilon$ accuracy will be $N = \sum_{k=1}^K m(k)$, where $m(k)$ is the number of inner iterations required at iteration $k$.

As already noted in the discussion of this subsection the AL function is comprised of a Lipschitz smooth function (the original cost) and a H\"older smooth function (the augmenting term). Moreover, the H\"older smooth part has a modulo of $H = \lambda \|A\|^q$. In every inner loop we require that $L_\lambda (x^{k+1}, y^k) - \inf L_\lambda(\cdot, y^k) \leq \varepsilon_k = \tfrac{c}{(k+1)^{p+1}}$. Therefore, from \cite[Theorem 1.1]{grimmer2023optimal} we have that each inner loop requires at most 
\begin{equation}
    m(k) = \lceil4(\tfrac{L(k+1)^{p+1}}{c+1})^{\tfrac{1}{2}}D^{\tfrac{1}{2}} + \tfrac{1+3q}{1+q}2^{\tfrac{3+q}{1+3q}}(\tfrac{H(k+1)^{p+1}}{c+1})^{\tfrac{2}{1+3q}}D^{\tfrac{1+q}{1+3q}}\rceil.
\end{equation}
We therefore obtain the following lower bound for the total number of iterations:
\begin{align*}
    N \geq \sum_{k=1}^K m(k) 
    &\geq 4(\tfrac{LD}{c+1})^{\tfrac{1}{2}}\sum_{k=1}^K (k+1)^{\tfrac{p+1}{2}} 
    + 
    \tfrac{1+3q}{1+q}2^{\tfrac{3+q}{1+3q}}(\tfrac{H}{c+1})^{\tfrac{2}{1+3q}}D^{\tfrac{1+q}{1+3q}}\sum_{k=1}^K (k+1)^{\tfrac{2(p+1)}{1+3q}}
    \\
    & \geq 4(\tfrac{LD}{c+1})^{\tfrac{1}{2}}f(K,\tfrac{p+1}{2})
    +
    \tfrac{1+3q}{1+q}2^{\tfrac{3+q}{1+3q}}(\tfrac{H}{c+1})^{\tfrac{2}{1+3q}}D^{\tfrac{1+q}{1+3q}}f(K, \tfrac{2(p+1)}{1+3q}),
\end{align*}
where $f(\cdot, \cdot)$ is Faulhaber's formula. Therefore we can see that $N = O((\tfrac{c+1}{\varepsilon})^{(\tfrac{2(p+1)}{1+3q}+1)q})$.
